SRG/eROSITA catalogue of X-ray active SDSS dwarf galaxies

We present a sample of 99 dwarf galaxies ($M_*<10^{9.5} M_\odot$) with X-ray activity in their central regions. The sample was obtained from a match of the SRG/eROSITA X-ray catalogue in the Eastern Galactic hemisphere with the MPA-JHU SDSS catalogue. The obtained matches were cleaned rigorously with the help of external optical catalogues to increase the purity of the sample. This work is the largest study of this kind -- X-ray activity in $\approx 85$ per cent of matched dwarfs was not reported before. The majority of X-ray active dwarfs are identified as star-forming galaxies. However, the X-ray luminosity of 82 objects cannot be explained by the collective emission of X-ray binaries, rendering them strong candidates for dwarf galaxies with an active accreting black hole in their centre. We find that the fraction of AGN among dwarf galaxies drops from $\sim 2\cdot 10^{-2}$ at $L_X\sim 10^{39}$ erg/s to $\sim (2-4)\cdot 10^{-4}$ at $L_X\sim 10^{41}$ erg/s and increases with the stellar mass of the host galaxy. We serendipitously discovered sources with unexpected properties. We report on a tidal disruption event (TDE) candidate in a dwarf galaxy, a massive black hole in a dwarf galaxy with a soft thermal spectrum, a luminous dwarf galaxy with an obscured X-ray spectrum and a few other peculiar sources. We found three Ultra-luminous X-ray source (ULX) candidates and a sample of X-ray bright galaxy pairs, in four of which both members shine in X-rays.

==> figures/table_only.tex <==
\begin{longtable}{llllllllllll}
\caption{eROSITA-detected dwarf galaxies} \label{tab:dwarfs} \\
\toprule
ID$^{(1)}$ & RA$^{(2)}$ & DEC$^{(3)}$ & Simbad$^{(4)}$ & $z$$^{(5)}$ & ID$_{\rm X}$$^{(6)}$ & RA$_{\rm X}$$^{(7)}$ & DEC$_{\rm X}$$^{(8)}$ & $\sigma_{\rm X}$$^{(9)}$ & $M_*, M_{\odot}$$^{(10)}$ & $L_{\rm X, 0.3-8}$ erg s$^{-1}$$^{(11)}$ & $\frac{L_{\rm X, 0.5-8}}{L_{\rm X, XRB}}$$^{(12)}$ \\
\midrule
\endfirsthead
\caption[]{eROSITA-selected dwarf galaxies} \\
\toprule
ID$^{(1)}$ & RA$^{(2)}$ & DEC$^{(3)}$ & Simbad$^{(4)}$ & $z$$^{(5)}$ & ID$_{\rm X}$$^{(6)}$ & RA$_{\rm X}$$^{(7)}$ & DEC$_{\rm X}$$^{(8)}$ & $\sigma_{\rm X}$$^{(9)}$ & $M_*, M_{\odot}$$^{(10)}$ & $L_{\rm X, 0.3-8}$ erg s$^{-1}$$^{(11)}$ & $\frac{L_{\rm X, 0.5-8}}{L_{\rm X, XRB}}$$^{(12)}$ \\
\midrule
\endhead
\midrule
\multicolumn{12}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
2349 & 253.88911 & 63.24213 & NGC  6275 & 0.023 & SRGe J165533.6+631432 & 253.88992 & 63.24216 & 5.8 & $2.1^{+1.1}_{-0.4}\times10^{9}$ & $3.4\pm0.7\times10^{40}$ & 3.1 \\
2364 & 253.90256 & 64.01973 & SDSSCGB 51726.2 & 0.023 & SRGe J165536.2+640107 & 253.90074 & 64.01858 & 5.6 & $5.5^{+2.2}_{-1.6}\times10^{7}$ & $1.7\pm0.7\times10^{40}$ & 302.4 \\
2399 & 255.30408 & 60.25146 & Z 299-45 & 0.013 & SRGe J170112.9+601459 & 255.30383 & 60.24964 & 7.3 & $1.04^{+0.25}_{-0.13}\times10^{9}$ & $4.0\pm1.8\times10^{39}$ & 1.8 \\
2448 & 260.10727 & 62.60368 & 2MASX J17202580+6236136 & 0.012 & SRGe J172025.5+623614 & 260.10636 & 62.604 & 6.1 & $2.33^{+0.6}_{-0.34}\times10^{9}$ & $6.4\pm1.4\times10^{39}$ & 2.0 \\
2506 & 262.31793 & 59.56275 & SDSS J172916.31+593346.0 & 0.018 & SRGe J172915.7+593345 & 262.31561 & 59.5625 & 6.4 & $2.0^{+0.34}_{-0.24}\times10^{8}$ & $1.3\pm0.4\times10^{40}$ & 19.9 \\
2539 & 259.19885 & 61.92012 & UGC 10796 & 0.01 & SRGe J171648.5+615513 & 259.20201 & 61.92032 & 7.4 & $1.45^{+0.28}_{-0.17}\times10^{9}$ & $4.6\pm1.1\times10^{39}$ & 1.3 \\
2556 & 262.07526 & 60.94234 & UGC 10880 & 0.013 & SRGe J172817.5+605630 & 262.07297 & 60.9416 & 8.5 & $1.22^{+0.5}_{-0.21}\times10^{6}$ & $5.8\pm1.7\times10^{39}$ & $4.988\times10^{3}$ \\
2595 & 257.75494 & 56.90007 & SDSS J171101.19+565400.2 & 0.028 & SRGe J171101.4+565401 & 257.75573 & 56.90038 & 7.2 & $6.9^{+1.6}_{-0.9}\times10^{8}$ & $2.3\pm1.1\times10^{40}$ & 24.6 \\
2824 & 261.03375 & 58.99508 & NGC  6373 & 0.011 & SRGe J172407.4+585940 & 261.03082 & 58.99438 & 9.0 & $1.99^{+0.5}_{-0.28}\times10^{9}$ & $2.3\pm1.3\times10^{39}$ & 1.1 \\
3474 & 7.71736 & 0.52872 & LEDA    1881 & 0.019 & SRGe J003051.9+003149 & 7.71617 & 0.53035 & 10.8 & $1.13^{+0.21}_{-0.13}\times10^{9}$ & $2.2\pm1.5\times10^{40}$ & 7.9 \\
4296 & 38.44556 & -1.02454 & SDSS J023346.93-010128.3 & 0.049 & SRGe J023346.8-010129 & 38.44505 & -1.02478 & 5.0 & $2.9^{+1.0}_{-0.6}\times10^{9}$ & $2.01\pm0.28\times10^{42}$ & 385.6 \\
5545 & 29.86125 & 14.83424 & LEDA 1468320 & $7.0\times10^{-3}$ & SRGe J015926.8+145002 & 29.86185 & 14.83388 & 5.4 & $2.52^{+0.5}_{-0.33}\times10^{8}$ & $4.1\pm0.9\times10^{40}$ & 123.5 \\
6328 & 147.17334 & 59.261 & Z 289-19 & $7.4\times10^{-3}$ & SRGe J094842.4+591548 & 147.17679 & 59.26339 & 13.6 & $2.0^{+0.5}_{-0.4}\times10^{9}$ & $1.1\pm0.4\times10^{40}$ & 2.9 \\
7394 & 195.00429 & 66.87216 & - & 0.048 & SRGe J130000.5+665216 & 195.00222 & 66.871 & 5.4 & $2.1^{+0.5}_{-0.35}\times10^{9}$ & $1.14\pm0.17\times10^{42}$ & 543.2 \\
9028 & 126.51829 & 45.96761 & UGC  4393 & $3.1\times10^{-3}$ & SRGe J082604.4+455805 & 126.5185 & 45.96799 & 6.6 & $1.37^{+0.35}_{-0.21}\times10^{9}$ & $5.4\pm1.0\times10^{39}$ & 1.5 \\
9225 & 143.50993 & 55.23978 & Mrk  116B & $2.6\times10^{-3}$ & SRGe J093402.0+551427 & 143.5085 & 55.24084 & 5.6 & $1.098^{+0.6}_{-0.03}\times10^{6}$ & $5.0\pm0.9\times10^{39}$ & 11.9 \\
10487 & 233.60663 & 4.1352 & [RGG2013] 123 & 0.04 & SRGe J153425.5+040806 & 233.60638 & 4.13505 & 5.0 & $2.5\pm0.7\times10^{9}$ & $9.3\pm1.2\times10^{41}$ & 222.0 \\
10619 & 173.33403 & 63.27942 & UGC  6534 & $4.1\times10^{-3}$ & SRGe J113320.8+631646 & 173.33667 & 63.2795 & 11.3 & $2.5^{+0.7}_{-0.4}\times10^{6}$ & $2.5\pm1.1\times10^{39}$ & $1.927\times10^{3}$ \\
11001 & 228.3716 & 58.50932 & Mrk  847 & $8.5\times10^{-3}$ & SRGe J151329.3+583035 & 228.37189 & 58.50971 & 9.0 & $2.6^{+0.7}_{-0.5}\times10^{9}$ & $3.4\pm1.6\times10^{39}$ & 1.4 \\
11048 & 233.80957 & 57.51482 & 2MASX J15351422+5730529 & 0.01 & SRGe J153513.7+573053 & 233.80694 & 57.51461 & 6.1 & $6.1^{+1.6}_{-0.9}\times10^{8}$ & $7.6\pm2.3\times10^{39}$ & 11.8 \\
11092 & 233.36633 & 53.51831 & SDSS J153327.91+533105.9 & 0.087 & SRGe J153326.8+533105 & 233.36171 & 53.51814 & 10.1 & $1.8^{+1.4}_{-0.6}\times10^{9}$ & $4.2\pm1.8\times10^{41}$ & 21.1 \\
11124 & 234.2674 & 55.26406 & SDSS J153704.18+551550.5 & $3.5\times10^{-3}$ & SRGe J153704.5+551550 & 234.26857 & 55.26376 & 5.0 & $7.7^{+1.5}_{-1.2}\times10^{6}$ & $1.79\pm0.17\times10^{40}$ & 113.8 \\
11195 & 237.02917 & 55.719 & NVSS J154806+554305 & 0.04 & SRGe J154806.7+554307 & 237.02774 & 55.71859 & 10.2 & $2.1^{+0.7}_{-0.4}\times10^{7}$ & $9.0\pm3.5\times10^{40}$ & 255.1 \\
11289 & 242.79799 & 48.33444 & 2MASX J16111153+4820036 & $9.4\times10^{-3}$ & SRGe J161111.5+482005 & 242.79792 & 48.33472 & 6.7 & $3.4^{+0.7}_{-0.4}\times10^{8}$ & $6.9\pm1.9\times10^{39}$ & 5.0 \\
11291 & 243.02216 & 48.8183 & - & 0.02 & SRGe J161205.4+484905 & 243.02259 & 48.8181 & 7.0 & $1.88^{+0.31}_{-0.21}\times10^{8}$ & $2.7\pm0.9\times10^{40}$ & 44.3 \\
11387 & 244.4016 & 46.082 & 2MASX J16173642+4604552 & 0.02 & SRGe J161737.2+460458 & 244.40506 & 46.0828 & 9.9 & $3.1^{+0.8}_{-0.4}\times10^{9}$ & $1.1\pm0.7\times10^{40}$ & 1.8 \\
11530 & 249.91254 & 43.29555 & MCG+07-34-128 & 0.016 & SRGe J163938.9+431741 & 249.91211 & 43.29459 & 12.2 & $1.94^{+0.4}_{-0.25}\times10^{9}$ & $1.5\pm0.6\times10^{40}$ & 5.2 \\
11568 & 250.23807 & 44.94012 & [VV2003c] J164057.1+445624 & 0.018 & SRGe J164056.8+445620 & 250.23652 & 44.93901 & 8.7 & $8.0^{+1.5}_{-1.3}\times10^{7}$ & $1.2\pm0.6\times10^{40}$ & 29.9 \\
11569 & 250.68242 & 45.71156 & LEDA 2269311 & 0.015 & SRGe J164243.4+454244 & 250.68074 & 45.71209 & 10.1 & $1.2^{+0.26}_{-0.16}\times10^{8}$ & $2.1\pm0.6\times10^{40}$ & 39.5 \\
11622 & 254.62193 & 40.95593 & SDSS J165829.26+405721.5 & 0.028 & SRGe J165829.7+405721 & 254.62361 & 40.95597 & 12.5 & $4.2^{+0.6}_{-0.5}\times10^{8}$ & $8.6\pm2.2\times10^{40}$ & 69.2 \\
11958 & 356.44275 & -8.78514 & LEDA  999228 & 0.056 & SRGe J234545.4-084707 & 356.43932 & -8.7854 & 12.6 & $2.16^{+0.5}_{-0.28}\times10^{9}$ & $3.6\pm2.0\times10^{41}$ & 69.1 \\
12509 & 26.14118 & -8.7731 & MCG-02-05-039 & 0.03 & SRGe J014433.6-084630 & 26.14016 & -8.77513 & 10.3 & $2.91^{+0.4}_{-0.3}\times10^{9}$ & $10\pm4.\times10^{40}$ & 9.1 \\
12608 & 32.92161 & -9.30599 & NGC   853 & $5.0\times10^{-3}$ & SRGe J021141.3-091817 & 32.92202 & -9.30458 & 11.2 & $3.4^{+0.5}_{-0.4}\times10^{6}$ & $3.3\pm1.0\times10^{39}$ & 454.7 \\
13693 & 336.8779 & -9.66499 & LEDA  988084 & $5.7\times10^{-3}$ & SRGe J222730.9-093959 & 336.87871 & -9.66634 & 7.2 & $2.6^{+0.7}_{-0.4}\times10^{7}$ & $8.8\pm3.1\times10^{39}$ & 13.2 \\
15429 & 206.67245 & 59.82294 & MCG+10-20-028 & $6.2\times10^{-3}$ & SRGe J134641.8+594925 & 206.67409 & 59.82353 & 8.9 & $5.1^{+1.3}_{-1.0}\times10^{8}$ & $3.7\pm1.5\times10^{39}$ & 15.2 \\
15677 & 232.06538 & 52.84361 & - & 0.019 & SRGe J152816.3+525041 & 232.06794 & 52.84466 & 8.7 & $2.6^{+0.7}_{-0.4}\times10^{8}$ & $1.9\pm1.3\times10^{40}$ & 38.1 \\
16640 & 42.39076 & 0.04646 & LEDA 1155772 & 0.186 & SRGe J024933.7+000245 & 42.39057 & 0.0458 & 11.3 & $1.3^{+1.5}_{-0.8}\times10^{8}$ & $1.22\pm0.28\times10^{43}$ & $4.48859\times10^{5}$ \\
18466 & 151.82887 & 47.00639 & UGC  5451 & $2.4\times10^{-3}$ & SRGe J100718.9+470020 & 151.82873 & 47.00552 & 9.6 & $1.2^{+0.28}_{-0.2}\times10^{8}$ & $1.1\pm0.4\times10^{39}$ & 16.4 \\
18549 & 164.24457 & 50.14062 & 2MASX J10565868+5008256 & $4.6\times10^{-3}$ & SRGe J105658.8+500828 & 164.24494 & 50.14115 & 6.7 & $1.06^{+0.4}_{-0.17}\times10^{8}$ & $5.6\pm1.5\times10^{39}$ & 23.3 \\
18900 & 187.5442 & 52.76308 & LEDA 2423061 & 0.06 & SRGe J123011.3+524543 & 187.54727 & 52.76196 & 8.5 & $2.6^{+1.3}_{-0.4}\times10^{9}$ & $5.9\pm2.3\times10^{41}$ & 157.7 \\
19521 & 158.13281 & 54.40104 & Mrk   33 & $9.8\times10^{-3}$ & SRGe J103232.0+542401 & 158.13351 & 54.40027 & 8.1 & $9.5^{+4.0}_{-1.7}\times10^{8}$ & $4.2\pm0.8\times10^{40}$ & 18.6 \\
20701 & 158.5423 & 58.06363 & Mrk 1434 & $7.5\times10^{-3}$ & SRGe J103410.1+580347 & 158.54189 & 58.0631 & 5.9 & $1.0^{+0.5}_{-0.04}\times10^{7}$ & $1.5\pm0.5\times10^{40}$ & 41.0 \\
20867 & 171.68462 & 59.15545 & IC  691 & $5.5\times10^{-3}$ & SRGe J112644.4+590921 & 171.68514 & 59.15595 & 8.0 & $9.3^{+4.0}_{-1.6}\times10^{8}$ & $1.37\pm0.26\times10^{40}$ & 4.9 \\
20929 & 176.93875 & 59.88667 & MCG+10-17-072 & $4.3\times10^{-3}$ & SRGe J114745.9+595304 & 176.94125 & 59.88458 & 10.0 & $1.7^{+0.8}_{-0.4}\times10^{8}$ & $2.4\pm1.0\times10^{39}$ & 5.5 \\
20944 & 184.00491 & 59.50806 & Mrk 1468 & 0.015 & SRGe J121601.4+593024 & 184.00592 & 59.50675 & 8.4 & $2.0^{+0.7}_{-0.4}\times10^{9}$ & $2.3\pm0.5\times10^{41}$ & 62.3 \\
21021 & 186.27255 & 61.15314 & SDSS J122505.40+610911.7 & $2.3\times10^{-3}$ & SRGe J122505.3+610912 & 186.27217 & 61.15329 & 6.8 & $8.5^{+2.4}_{-0.5}\times10^{6}$ & $1.27\pm0.31\times10^{39}$ & 3.7 \\
21115 & 197.96373 & 60.24735 & UGC  8282 & 0.011 & SRGe J131151.3+601455 & 197.96392 & 60.24863 & 8.4 & $3.3^{+0.5}_{-0.4}\times10^{8}$ & $1.5\pm0.6\times10^{40}$ & 26.5 \\
21456 & 176.48587 & 50.19979 & NGC  3870 & $4.0\times10^{-3}$ & SRGe J114557.0+501209 & 176.48763 & 50.2025 & 17.4 & $5.2^{+1.2}_{-1.3}\times10^{8}$ & $1.8\pm0.8\times10^{39}$ & 2.7 \\
22648 & 167.01215 & 53.61681 & UGC  6182 & $4.1\times10^{-3}$ & SRGe J110803.3+533700 & 167.01393 & 53.61657 & 9.1 & $1.17^{+0.26}_{-0.16}\times10^{6}$ & $4.4\pm1.6\times10^{39}$ & $1.854\times10^{3}$ \\
22933 & 183.35844 & 54.60879 & SDSS J121326.03+543631.7 & $8.0\times10^{-3}$ & SRGe J121325.9+543632 & 183.35809 & 54.60893 & 7.3 & $2.43^{+0.4}_{-0.28}\times10^{7}$ & $1.5\pm0.4\times10^{40}$ & 161.7 \\
23630 & 320.71609 & -0.99672 & SDSS J212252.00-005949.4 & 0.184 & SRGe J212252.0-005957 & 320.71659 & -0.99911 & 9.3 & $2.82^{+0.5}_{-0.32}\times10^{9}$ & $1.8\pm0.5\times10^{43}$ & 859.9 \\
25180 & 214.87833 & 51.92448 & MCG+09-23-060 & 0.029 & SRGe J141931.2+515528 & 214.88 & 51.92432 & 7.4 & $2.76^{+0.5}_{-0.35}\times10^{9}$ & $1.36\pm0.34\times10^{41}$ & 87.8 \\
25225 & 221.83762 & 48.90128 & 2MASX J14472098+4854050 & $7.4\times10^{-3}$ & SRGe J144721.0+485403 & 221.8377 & 48.90079 & 8.4 & $6.4^{+3.1}_{-1.4}\times10^{8}$ & $3.2\pm1.5\times10^{39}$ & 2.5 \\
25312 & 225.3539 & 48.10772 & 2MASX J15012488+4806276 & 0.011 & SRGe J150125.2+480628 & 225.35481 & 48.10766 & 7.8 & $5.9^{+2.3}_{-1.2}\times10^{8}$ & $3.4\pm1.7\times10^{39}$ & 2.5 \\
25337 & 228.05357 & 47.27519 & LEDA   87385 & 0.053 & SRGe J151212.9+471635 & 228.05386 & 47.27634 & 8.7 & $1.31^{+0.4}_{-0.26}\times10^{9}$ & $2.3\pm0.8\times10^{41}$ & 3.8 \\
27238 & 227.16699 & 52.45378 & Mrk  846 & 0.011 & SRGe J150840.4+522713 & 227.16818 & 52.45371 & 6.9 & $1.90^{+0.5}_{-0.28}\times10^{9}$ & $4.7\pm1.2\times10^{40}$ & 19.5 \\
28027 & 139.34045 & 41.91099 & UGC  4904 & $5.6\times10^{-3}$ & SRGe J091721.1+415439 & 139.33812 & 41.91083 & 8.8 & $1.09^{+0.28}_{-0.12}\times10^{6}$ & $6.3\pm2.5\times10^{39}$ & $9.937\times10^{3}$ \\
30754 & 180.76497 & 56.91676 & LEDA 2551818 & 0.019 & SRGe J120303.9+565500 & 180.76619 & 56.91658 & 7.0 & $2.7^{+0.7}_{-0.5}\times10^{9}$ & $1.16\pm0.26\times10^{41}$ & 79.1 \\
30769 & 182.85503 & 58.75883 & SBSG 1209+590 & 0.011 & SRGe J121124.6+584540 & 182.85253 & 58.76102 & 9.4 & $3.9^{+0.5}_{-0.4}\times10^{8}$ & $1.7\pm0.6\times10^{40}$ & 8.5 \\
30874 & 200.21776 & 57.64159 & NGC  5109 & $7.0\times10^{-3}$ & SRGe J132053.1+573833 & 200.22106 & 57.64258 & 8.1 & $1.1^{+1.1}_{-0.7}\times10^{9}$ & $7.4\pm2.3\times10^{39}$ & 20.6 \\
30902 & 201.47424 & 57.25445 & Mrk   66 & 0.021 & SRGe J132554.2+571518 & 201.47571 & 57.25493 & 10.2 & $1.90^{+0.21}_{-0.18}\times10^{9}$ & $5.7\pm2.3\times10^{40}$ & 7.2 \\
31488 & 241.44122 & 41.34475 & Mrk 1104 & $7.5\times10^{-3}$ & SRGe J160545.5+412039 & 241.4394 & 41.34426 & 6.2 & $5.3\pm0.6\times10^{8}$ & $5.2\pm1.4\times10^{39}$ & 1.5 \\
31794 & 216.3376 & 39.53958 & UGC  9242 & $5.5\times10^{-3}$ & SRGe J142521.3+393223 & 216.33894 & 39.5397 & 9.4 & $2.9^{+0.6}_{-0.4}\times10^{8}$ & $2.8\pm1.0\times10^{39}$ & 6.7 \\
31817 & 216.90254 & 41.25776 & NGC  5630 & $7.0\times10^{-3}$ & SRGe J142737.4+411529 & 216.90603 & 41.25813 & 11.1 & $2.5^{+0.5}_{-0.31}\times10^{9}$ & $2.5\pm1.4\times10^{39}$ & 0.8 \\
32206 & 166.28383 & 44.74646 & [BKD2008] WR 276 & 0.022 & SRGe J110508.3+444455 & 166.28462 & 44.74856 & 9.3 & $4.9^{+0.6}_{-0.7}\times10^{8}$ & $7.3\pm2.9\times10^{40}$ & 3.4 \\
32658 & 206.99294 & 39.38945 & LEDA 2148943 & $9.3\times10^{-3}$ & SRGe J134758.2+392325 & 206.99243 & 39.39034 & 8.8 & $9.4^{+2.1}_{-1.2}\times10^{7}$ & $5.4\pm2.7\times10^{39}$ & 32.5 \\
33466 & 253.33936 & 23.08278 & SDSS J165321.44+230458.0 & 0.036 & SRGe J165321.9+230500 & 253.34143 & 23.08311 & 9.8 & $3.0^{+0.7}_{-0.4}\times10^{9}$ & $1.5\pm0.7\times10^{41}$ & 38.8 \\
33862 & 159.65518 & 44.52309 & FIRST J103837.1+443123 & 0.012 & SRGe J103837.6+443121 & 159.6566 & 44.5225 & 9.3 & $1.3^{+0.9}_{-0.4}\times10^{9}$ & $1.9\pm1.1\times10^{40}$ & 1.2 \\
34306 & 177.55119 & 42.0745 & UGC  6805 & $3.9\times10^{-3}$ & SRGe J115012.4+420427 & 177.5515 & 42.07431 & 10.1 & $4.1^{+1.0}_{-0.7}\times10^{8}$ & $2.1\pm0.9\times10^{39}$ & 4.9 \\
34352 & 177.94843 & 48.68314 & NGC  3928 & $3.9\times10^{-3}$ & SRGe J115147.4+484100 & 177.94769 & 48.68317 & 8.6 & $2.3^{+0.6}_{-0.5}\times10^{9}$ & $3.3\pm1.0\times10^{39}$ & 2.2 \\
34500 & 181.94214 & 43.12635 & NGC  4117 & $4.7\times10^{-3}$ & SRGe J120746.3+430733 & 181.94302 & 43.12581 & 9.7 & $2.2^{+0.5}_{-0.4}\times10^{9}$ & $2.7\pm1.2\times10^{39}$ & 4.9 \\
37144 & 41.71429 & -0.48567 & - & 0.044 & SRGe J024651.9-002909 & 41.71637 & -0.48585 & 8.4 & $1.3^{+2.0}_{-1.0}\times10^{9}$ & $2.0\pm0.9\times10^{41}$ & 746.5 \\
39439 & 215.28319 & 35.29539 & MCG+06-32-004 & 0.012 & SRGe J142108.6+351741 & 215.28596 & 35.29464 & 9.8 & $2.9^{+1.5}_{-0.4}\times10^{8}$ & $1.2\pm0.5\times10^{40}$ & 3.3 \\
39591 & 230.56068 & 31.47515 & Mrk  850 & $7.3\times10^{-3}$ & SRGe J152214.7+312832 & 230.56111 & 31.47566 & 6.5 & $2.2^{+1.4}_{-0.7}\times10^{7}$ & $7.5\pm1.9\times10^{39}$ & 13.7 \\
39612 & 233.70477 & 28.65526 & NGC  5958 & $6.7\times10^{-3}$ & SRGe J153449.4+283916 & 233.70602 & 28.65434 & 10.4 & $2.7^{+0.8}_{-0.5}\times10^{9}$ & $6.4\pm1.7\times10^{39}$ & 1.9 \\
39731 & 242.73491 & 23.99648 & SDSS J161056.37+235947.3 & 0.033 & SRGe J161056.1+235950 & 242.73375 & 23.99715 & 8.0 & $1.4^{+1.7}_{-1.0}\times10^{9}$ & $1.6\pm0.5\times10^{41}$ & 527.9 \\
39846 & 49.62766 & 40.50241 & LEDA 2166728 & 0.026 & SRGe J031830.3+403004 & 49.62641 & 40.50113 & 10.4 & $1.01^{+0.18}_{-0.12}\times10^{9}$ & $9.\pm4.\times10^{40}$ & 51.8 \\
41568 & 229.95583 & 8.07313 & SDSS J151949.39+080423.2 & 0.042 & SRGe J151949.8+080428 & 229.95769 & 8.07432 & 7.9 & $1.83^{+0.4}_{-0.28}\times10^{9}$ & $2.4\pm0.9\times10^{41}$ & 111.7 \\
43461 & 137.56142 & 59.95417 & UGC  4808 & $4.4\times10^{-3}$ & SRGe J091015.0+595710 & 137.56234 & 59.95288 & 6.5 & $2.7^{+0.6}_{-0.5}\times10^{8}$ & $7.5\pm1.6\times10^{39}$ & 115.3 \\
44628 & 231.65569 & 6.99491 & 2MASS J15263736+0659417 & 0.038 & SRGe J152637.5+065942 & 231.65612 & 6.99489 & 5.0 & $2.6^{+0.9}_{-0.7}\times10^{9}$ & $5.02\pm0.26\times10^{42}$ & 777.2 \\
45689 & 313.08316 & 0.05463 & - & 0.211 & SRGe J205220.2+000319 & 313.08396 & 0.05528 & 6.7 & $5.^{+25}_{-5.}\times10^{8}$ & $9.1\pm1.9\times10^{43}$ & $8.59861\times10^{5}$ \\
47785 & 203.8987 & 29.21744 & UGC  8578 & $4.1\times10^{-3}$ & SRGe J133535.6+291306 & 203.89854 & 29.21821 & 5.0 & $1.45^{+0.29}_{-0.26}\times10^{6}$ & $6.6\pm1.1\times10^{39}$ & $1.471\times10^{3}$ \\
49241 & 186.45361 & 33.54687 & NGC  4395 & $1.0\times10^{-3}$ & SRGe J122548.6+333247 & 186.45266 & 33.54625 & 7.2 & $2.5^{+0.7}_{-0.5}\times10^{7}$ & $1.04\pm0.28\times10^{39}$ & 191.9 \\
49754 & 196.48788 & 32.839 & LEDA 2014266 & 0.018 & SRGe J130557.6+325013 & 196.49004 & 32.83702 & 14.0 & $6.7^{+1.0}_{-0.7}\times10^{8}$ & $3.0\pm1.5\times10^{40}$ & 17.7 \\
50706 & 176.60869 & 34.85195 & Mrk  429 & $5.8\times10^{-3}$ & SRGe J114625.8+345105 & 176.60744 & 34.85128 & 14.8 & $2.6^{+0.6}_{-0.4}\times10^{7}$ & $3.5\pm2.0\times10^{39}$ & 53.4 \\
50842 & 205.80479 & 36.74931 & 2MASX J13431319+3644574 & 0.02 & SRGe J134313.2+364455 & 205.80521 & 36.74859 & 5.9 & $1.87^{+0.70}_{-0.34}\times10^{9}$ & $1.71\pm0.24\times10^{41}$ & 25.4 \\
50909 & 201.08405 & 36.59609 & Mrk  451 & 0.016 & SRGe J132419.9+363552 & 201.08301 & 36.59783 & 11.1 & $2.2^{+1.2}_{-0.6}\times10^{9}$ & $8.1\pm3.2\times10^{40}$ & 6.9 \\
51004 & 200.30437 & 31.22184 & UGC  8392 & 0.017 & SRGe J132113.0+311303 & 200.30419 & 31.21747 & 16.1 & $2.9^{+0.6}_{-0.4}\times10^{9}$ & $10\pm4.\times10^{40}$ & 91.8 \\
51224 & 204.60362 & 33.11771 & UGC  8630 & $6.8\times10^{-3}$ & SRGe J133824.9+330704 & 204.60384 & 33.11785 & 8.9 & $8.6^{+6.0}_{-2.9}\times10^{8}$ & $5.1\pm1.8\times10^{39}$ & 1.2 \\
52047 & 217.16235 & 30.63451 & Z 163-59 & 0.013 & SRGe J142838.7+303809 & 217.16116 & 30.63569 & 9.7 & $1.43^{+0.4}_{-0.26}\times10^{9}$ & $5.1\pm1.7\times10^{40}$ & 33.4 \\
52077 & 217.22009 & 27.8344 & 2MASS J14285283+2750037 & 0.016 & SRGe J142852.8+275005 & 217.2198 & 27.83462 & 8.8 & $1.12^{+0.23}_{-0.14}\times10^{9}$ & $1.4\pm0.8\times10^{40}$ & 7.2 \\
52695 & 227.23254 & 25.73327 & UGC  9739 & $7.3\times10^{-3}$ & SRGe J150856.4+254359 & 227.23492 & 25.73296 & 11.3 & $7.4^{+1.2}_{-0.7}\times10^{7}$ & $5.1\pm1.8\times10^{39}$ & 24.1 \\
53431 & 241.38271 & 17.80728 & 2XMM J160531.8+174825 & 0.032 & SRGe J160531.8+174824 & 241.38247 & 17.80677 & 6.9 & $1.64^{+0.4}_{-0.31}\times10^{9}$ & $2.8\pm0.7\times10^{41}$ & 224.9 \\
57825 & 162.58224 & 48.33294 & - & 0.098 & SRGe J105019.2+481958 & 162.58002 & 48.33282 & 11.0 & $7.5^{+2.7}_{-1.2}\times10^{8}$ & $1.1\pm0.6\times10^{42}$ & 258.3 \\
63593 & 213.63451 & 17.98318 & ECO 2507 & 0.024 & SRGe J141432.4+175900 & 213.63489 & 17.98327 & 9.5 & $1.43^{+0.17}_{-0.15}\times10^{8}$ & $5.6\pm2.3\times10^{40}$ & 9.9 \\
63898 & 233.69412 & 12.44725 & LEDA 3091021 & $9.0\times10^{-3}$ & SRGe J153446.8+122654 & 233.69496 & 12.44838 & 9.1 & $9.6^{+1.2}_{-0.9}\times10^{7}$ & $1.4\pm0.4\times10^{40}$ & 37.6 \\
64321 & 233.64713 & 15.20097 & NGC  5954 & $7.5\times10^{-3}$ & SRGe J153435.1+151203 & 233.64612 & 15.20094 & 9.0 & $7.9^{+7.0}_{-3.0}\times10^{6}$ & $1.08\pm0.31\times10^{40}$ & 40.5 \\
64653 & 234.13292 & 16.44037 & UGC  9925 & 0.011 & SRGe J153632.1+162628 & 234.13383 & 16.44113 & 5.6 & $6.8^{+1.7}_{-1.2}\times10^{8}$ & $4.4\pm0.8\times10^{40}$ & 163.3 \\
65319 & 240.86063 & 19.16268 & Mrk  296 & 0.016 & SRGe J160326.5+190940 & 240.86027 & 19.16108 & 7.7 & $2.1^{+2.1}_{-1.3}\times10^{9}$ & $2.1\pm0.9\times10^{40}$ & 22.7 \\


 \caption{(1) - ID of a dwarf; (2,3) - SDSS fiber coordinates in deg, (4) Galaxy name from Simbad; (5) redshift; (6,7,8) eROSITA name, coordinates (in deg); (9) eROSITA positional error in arcsec ; (10) Stellar mass (solar masses); (11)  X-ray luminosity in the 0.3--8 keV energy range (erg/s); (12) ratio of the observed X-ray luminosity to the expected X-ray binary emission (0.5--8 keV).}
\end{longtable}

